Random Walk-steered Majority Undersampling

In this work, we propose Random Walk-steered Majority Undersampling (RWMaU), which undersamples the majority points of a class imbalanced dataset, in order to balance the classes. Rather than marking the majority points which belong to the neighborhood of a few minority points, we are interested to perceive the closeness of the majority points to the minority class. Random walk, a powerful tool for perceiving the proximities of connected points in a graph, is used to identify the majority points which lie close to the minority class of a class-imbalanced dataset. The visit frequencies and the order of visits of the majority points in the walks enable us to perceive an overall closeness of the majority points to the minority class. The ones lying close to the minority class are subsequently undersampled. Empirical evaluation on 21 datasets and 3 classifiers demonstrate substantial improvement in performance of RWMaU over the competing methods.

==> RWMaU_ICONIP2021 Paper/tables/auc_tab.tex <==
\begin{tabular}{l|llllll|llllll|llllll}
\hline 
 & \multicolumn{6}{c|}{KNN} & \multicolumn{6}{c|}{C4.5} & \multicolumn{6}{c}{C4.5 + Bagging}\tabularnewline
\hline 
              & RWMaU   & Original   & RUS        & IHT        & CC         & NCR        & RWMaU   & Original   & RUS        & IHT        & CC         & NCR        & RWMaU & Original & RUS & IHT & CC & NCR\tabularnewline
\hline                                                        
yeast5        & 0.9871 (2) & 0.9830 (4) & 0.9735 (5) & 0.8497 (6) & 0.9868 (3) & \textbf{0.9909 (1)} & 0.9489 (3) & 0.8422 (5) & 0.9721 (2) & 0.8382 (6) & \textbf{0.9767 (1)} & 0.8647 (4) & 0.9837 (2) & 0.9548 (4) & 0.9828 (3) & 0.9241 (6) & \textbf{0.9876 (1)} & 0.9479 (5) \tabularnewline
yeast1289v7   & 0.7214 (2) & 0.6971 (3) & 0.6480 (5) & 0.5867 (6) & \textbf{0.7510 (1)} & 0.6804 (4) & \textbf{0.6051 (1)} & 0.5653 (4) & 0.5441 (6) & 0.5845 (3) & 0.5889 (2) & 0.5465 (5) & 0.6894 (3) & 0.6896 (2) & \textbf{0.7001} (1) & 0.5799 (6) & 0.6300 (5) & 0.6598 (4) \tabularnewline
wine-red-4    & 0.5871 (3) & 0.4987 (6) & 0.5765 (4) & 0.6048 (2) & \textbf{0.6321 (1)} & 0.5202 (5) & 0.5970 (2) & 0.5500 (5) & \textbf{0.6027 (1)} & 0.5325 (6) & 0.5902 (3) & 0.5585 (4) & \textbf{0.7574 (1)} & 0.6684 (5) & 0.6966 (3) & 0.6148 (6) & 0.6816 (4) & 0.7355 (2) \tabularnewline
yeast4        & 0.8481 (3) & 0.7755 (5) & 0.8906 (2) & 0.7179 (6) & \textbf{0.9094 (1)} & 0.8226 (4) & 0.7902 (2) & 0.6505 (5) & \textbf{0.8122 (1)} & 0.5825 (6) & 0.7119 (3) & 0.6899 (4) & \textbf{0.8900 (1)} & 0.7932 (5) & 0.8805 (2) & 0.6552 (6) & 0.8195 (4) & 0.8456 (3) \tabularnewline
yeast1458v7   & \textbf{0.6934 (1)} & 0.6233 (5) & 0.6079 (6) & 0.6479 (3) & 0.6535 (2) & 0.6338 (4) & \textbf{0.5645 (1)} & 0.4994 (6) & 0.5604 (2) & 0.5352 (3) & 0.5290 (4) & 0.5260 (5) & 0.6168 (4) & 0.6719 (2) & 0.6314 (3) & 0.5689 (5) & 0.5550 (6) & \textbf{0.7128 (1)} \tabularnewline
abalone9-18   & \textbf{0.7748 (1)} & 0.7307 (3) & 0.7092 (5) & 0.6271 (6) & 0.7131 (4) & 0.7328 (2) & \textbf{0.6813 (1)} & 0.6691 (3) & 0.6541 (5) & 0.5577 (6) & 0.6667 (4) & 0.6754 (2) & \textbf{0.8239 (1)} & 0.8105 (3) & 0.7979 (4) & 0.6057 (6) & 0.7787 (5) & 0.8107 (2) \tabularnewline
ecoli4        & \textbf{0.9963 (1)} & 0.9846 (5) & 0.9899 (3) & 0.9155 (6) & 0.9962 (2) & 0.9848 (4) & 0.8440 (2) & 0.8264 (5) & 0.8391 (3) & 0.8357 (4) & \textbf{0.8577 (1)} & 0.8123 (6) & \textbf{0.9315 (1)} & 0.9055 (5) & 0.9228 (3) & 0.9239 (2) & 0.9177 (4) & 0.8535 (6) \tabularnewline
led02456789v1 & 0.7555 (5) & 0.7635 (4) & 0.8205 (2) & \textbf{0.8389 (1)} & 0.7544 (6) & 0.7683 (3) & \textbf{0.6924 (1)} & 0.5726 (6) & 0.6103 (3) & 0.6277 (2) & 0.6087 (4) & 0.5809 (5) & 0.7497 (2) & 0.7206 (4) & 0.7177 (6) & 0.7180 (5) & \textbf{0.7712 (1)} & 0.7231 (3) \tabularnewline
page-blocks0  & \textbf{0.9586 (1)} & 0.9377 (4) & 0.9473 (2) & 0.5770 (6) & 0.9132 (5) & 0.9429 (3) & 0.9343 (2) & 0.8994 (4) & \textbf{0.9407 (1)} & 0.5874 (6) & 0.8752 (5) & 0.9292 (3) & 0.9703 (4) & 0.9721 (3) & \textbf{0.9798 (1)} & 0.5933 (6) & 0.9348 (5) & 0.9761 (2) \tabularnewline
ecoli3        & \textbf{0.9363 (1)} & 0.9265 (4) & 0.9301 (2) & 0.8329 (6) & 0.9232 (5) & 0.9273 (3) & \textbf{0.8264 (1)} & 0.7664 (6) & 0.7957 (4) & 0.7807 (5) & 0.8168 (2) & 0.7970 (3) & 0.8878 (4) & 0.8825 (6) & 0.8931 (3) & 0.8984 (2) & \textbf{0.9099 (1)} & 0.8863 (5) \tabularnewline
yeast3        & \textbf{0.9586 (1)} & 0.9407 (5) & 0.9463 (3) & 0.8716 (6) & 0.9574 (2) & 0.9462 (4) & \textbf{0.8969} (1) & 0.8223 (6) & 0.8931 (3) & 0.8268 (5) & 0.8966 (2) & 0.8852 (4) & 0.9588 (2) & 0.9410 (5) & \textbf{0.9608 (1)} & 0.9021 (6) & 0.9557 (3) & 0.9522 (4) \tabularnewline
new-thyroid1  & 0.9897 (3) & 0.9927 (2) & 0.9866 (4) & 0.9109 (6) & 0.9845 (5) & \textbf{0.9966 (1)} & 0.9462 (2) & 0.8857 (4) & 0.9461 (3) & 0.8418 (6) & \textbf{0.9474 (1)} & 0.8856 (5) & 0.9854 (3) & 0.9814 (4) & \textbf{0.9904 (1)} & 0.9624 (5) & 0.9882 (2) & 0.9436 (6) \tabularnewline
new-thyroid2  & 0.9724 (5) & \textbf{0.9977 (1)} & 0.9808 (4) & 0.8940 (6) & 0.9858 (3) & 0.9919 (2) & \textbf{0.9593 (1)} & 0.9158 (4) & 0.9172 (3) & 0.8751 (6) & 0.9420 (2) & 0.8920 (5) & 0.9955 (2) & \textbf{0.9965 (1)} & 0.9886 (3) & 0.9785 (6) & 0.9877 (4) & 0.9814 (5) \tabularnewline
vehicle3      & \textbf{0.7816 (1)} & 0.7742 (4) & 0.7653 (5) & 0.7758 (3) & 0.7578 (6) & 0.7788 (2) & 0.7446 (2) & 0.6855 (6) & 0.7046 (3) & \textbf{0.7514 (1)} & 0.6882 (5) & 0.7024 (4) & 0.8110 (4) & 0.8180 (2) & 0.8043 (6) & 0.8107 (5) & 0.8143 (3) & \textbf{0.8278 (1)} \tabularnewline
vehicle1      & \textbf{0.7735 (1)} & 0.7578 (4) & 0.7458 (6) & 0.7679 (2) & 0.7469 (5) & 0.7621 (3) & \textbf{0.7673} (1) & 0.6668 (6) & 0.6998 (4) & 0.7427 (3) & 0.6777 (5) & \textbf{0.7432 (2)} & 0.8310 (2) & 0.8191 (5) & 0.8214 (4) & \textbf{0.8325} (1) & 0.8052 (6) & 0.8272 (3) \tabularnewline
vehicle2      & 0.9485 (2) & \textbf{0.9600 (1)} & 0.9307 (5) & 0.9120 (6) & 0.9468 (3) & 0.9460 (4) & \textbf{0.9413 (1)} & 0.9286 (4) & 0.9213 (5) & 0.8945 (6) & 0.9385 (2) & 0.9340 (3) & 0.9861 (4) & 0.9862 (3) & \textbf{0.9884 (1)} & 0.9494 (6) & 0.9779 (5) & 0.9868 (2) \tabularnewline
glass0        & \textbf{0.8682 (1)} & 0.8491 (3) & 0.8539 (2) & 0.7704 (6) & 0.8463 (4) & 0.8423 (5) & 0.8094 (2) & \textbf{0.8373 (1)} & 0.7931 (4) & 0.7386 (6) & 0.7392 (5) & 0.8060 (3) & 0.8795 (3) & \textbf{0.9239 (1)} & 0.8894 (2) & 0.7866 (6) & 0.8531 (5) & 0.8672 (4) \tabularnewline
pima          & 0.7632 (2) & 0.7288 (6) & 0.7604 (3) & \textbf{0.7822 (1)} & 0.7451 (5) & 0.7598 (4) & 0.6114 (2) & 0.5606 (5) & 0.5659 (4) & \textbf{0.6217 (1)} & 0.5461 (6) & 0.6036 (3) & \textbf{0.6820 (1)} & 0.6404 (5) & 0.6476 (4) & 0.6728 (2) & 0.5624 (6) & 0.6650 (3) \tabularnewline
glass1        & 0.8702 (2) & \textbf{0.8844 (1)} & 0.8417 (5) & 0.7988 (6) & 0.8607 (3) & 0.8521 (4) & \textbf{0.7365 (1)} & 0.6946 (5) & 0.7054 (2) & 0.6258 (6) & 0.6966 (4) & 0.7006 (3) & 0.8392 (2) & \textbf{0.8404 (1)} & 0.8119 (4) & 0.6814 (6) & 0.8082 (5) & 0.8139 (3) \tabularnewline
wdbc          & 0.9519 (1) & 0.9454 (5) & 0.9497 (4) & 0.9504 (2) & 0.9500 (3) & 0.9431 (6) & \textbf{0.9372 (1)} & 0.9291 (2) & 0.9239 (4) & 0.9087 (6) & 0.9189 (5) & 0.9276 (3) & 0.9803 (5) & \textbf{0.9855 (1)} & 0.9840 (2) & 0.9712 (6) & 0.9826 (3) & 0.9809 (4) \tabularnewline
spam          & \textbf{0.8630 (1)} & 0.8580 (2) & 0.8503 (4) & 0.8499 (5) & 0.8510 (3) & 0.8458 (6) & \textbf{0.9069 (1)} & 0.9011 (2) & 0.8927 (4) & 0.8672 (6) & 0.8964 (3) & 0.8885 (5) & 0.9712 (2) & 0.9692 (4) & 0.9694 (3) & 0.9539 (6) & \textbf{0.9724 (1)} & 0.9644 (5) \tabularnewline
\hline        
Avg. rank              & 1.90       & 3.67       & 3.86       & 4.62       & 3.43       & 3.52       & 1.48       & 4.48       & 3.19       & 4.71       & 3.29       & 3.86       & 2.52       & 3.38       & 2.86       & 5.00       & 3.76       & 3.48       \tabularnewline
\hline 
\end{tabular}




        








==> RWMaU_ICONIP2021 Paper/tables/ds_desciption.tex <==
\begin{tabular}{lrrr}
  \hline
                &    n & d  & Imb. Ratio \\ 
  \hline                               
  yeast5        & 1484 & 8  & 32.73     \\ 
  yeast1289v7   & 947  & 8  & 30.57     \\ 
  wine-red-4    & 1599 & 11 & 29.17     \\ 
  yeast4        & 1484 & 8  & 28.10     \\ 
  yeast1458v7   & 693  & 8  & 22.10     \\ 
  abalone9-18   & 731  & 8  & 16.40     \\ 
  ecoli4        & 336  & 7  & 15.80     \\ 
  led02456789v1 & 443  & 7  & 10.97     \\ 
  page-blocks0  & 5472 & 10 & 8.79      \\ 
  ecoli3        & 336  & 7  & 8.60      \\ 
  yeast3        & 1484 & 8  & 8.10      \\ 
  new-thyroid1  & 215  & 5  & 5.14      \\ 
  new-thyroid2  & 215  & 5  & 5.14      \\ 
  vehicle3      & 846  & 18 & 2.99      \\ 
  vehicle1      & 846  & 18 & 2.90      \\ 
  vehicle2      & 846  & 18 & 2.88      \\ 
  glass0        & 214  & 9  & 2.06      \\ 
  pima          & 768  & 8  & 1.87      \\ 
  glass1        & 214  & 9  & 1.82      \\ 
  wdbc          & 569  & 30 & 1.68      \\ 
  spam          & 4597 & 57 & 1.54      \\ 
   \hline
\end{tabular}

==> RWMaU_ICONIP2021 Paper/tables/ds_description_transpose.tex <==
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrr}
  \hline
 & new-thyroid1 & pima & yeast4 & glass1 & vehicle3 & glass0 & ecoli3 & ecoli4 & vehicle1 & wdbc & new-thyroid2 & yeast1458v7 & yeast5 & yeast3 & vehicle2 & abalone9-18 & led02456789v1 & page-blocks0 & spam & yeast1289v7 & wine-red-4 \\ 
  \hline
n & 215.00 & 768.00 & 1484.00 & 214.00 & 846.00 & 214.00 & 336.00 & 336.00 & 846.00 & 569.00 & 215.00 & 693.00 & 1484.00 & 1484.00 & 846.00 & 731.00 & 443.00 & 5472.00 & 4597.00 & 947.00 & 1599.00 \\ 
  d & 5.00 & 8.00 & 8.00 & 9.00 & 18.00 & 9.00 & 7.00 & 7.00 & 18.00 & 30.00 & 5.00 & 8.00 & 8.00 & 8.00 & 18.00 & 8.00 & 7.00 & 10.00 & 57.00 & 8.00 & 11.00 \\ 
  imb.ratio & 5.14 & 1.87 & 28.10 & 1.82 & 2.99 & 2.06 & 8.60 & 15.80 & 2.90 & 1.68 & 5.14 & 22.10 & 32.73 & 8.10 & 2.88 & 16.40 & 10.97 & 8.79 & 1.54 & 30.57 & 29.17 \\ 
   \hline
\end{tabular}


==> RWMaU_ICONIP2021 Paper/tables/f1_tab.tex <==

\begin{tabular}{l|llllll|llllll|llllll}
\hline 
 & \multicolumn{6}{c|}{KNN} & \multicolumn{6}{c|}{C4.5} & \multicolumn{6}{c}{C4.5 + Bagging}\tabularnewline
\hline 
                & RWMaU   & Original     & RUS        & IHT        & CC         & NCR          & RWMaU   & Original   & RUS        & IHT        & CC         & NCR        & RWMaU  & Original & RUS & IHT & CC & NCR\tabularnewline
\hline 
yeast5          & 0.6200 (3) & 0.6606 (2.0) & 0.3978 (5) & 0.1420 (6) & 0.4052 (4) & \textbf{0.7540 (1.0)} & 0.4662 (5) & \textbf{0.6995 (1)} & 0.5478 (4) & 0.1726 (6) & 0.6000 (3) & 0.6470 (2) & 0.4699 (5) & 0.6760 (2) & 0.5128 (4) & 0.1972 (6) & 0.5647 (3) & \textbf{0.7272 (1)} \tabularnewline
yeast1289v7     & \textbf{0.1938 (1)} & 0.0000 (5.5) & 0.0930 (3) & 0.0760 (4) & 0.1064 (2) & 0.0000 (5.5) & \textbf{0.1953 (1)} & 0.1680 (2) & 0.0795 (6) & 0.0856 (5) & 0.0886 (4) & 0.1316 (3) & 0.1688 (3) & \textbf{0.2052 (1)} & 0.1274 (4) & 0.0786 (6) & 0.0904 (5) & 0.1821 (2) \tabularnewline
wine-red-4      & \textbf{0.1345 (1)} & 0.0000 (6.0) & 0.0898 (4) & 0.0924 (3) & 0.0952 (2) & 0.0787 (5.0) & \textbf{0.1652 (1)} & 0.1235 (3) & 0.1023 (4) & 0.0782 (6) & 0.0897 (5) & 0.1246 (2) & \textbf{0.1452 (1)} & 0.0897 (4) & 0.1318 (2) & 0.0791 (5) & 0.1004 (3) & 0.0438 (6) \tabularnewline
yeast4          & \textbf{0.4530 (1)} & 0.1616 (5.0) & 0.2824 (4) & 0.1148 (6) & 0.3137 (3) & 0.4200 (2.0) & 0.1943 (4) & 0.2751 (2) & 0.2164 (3) & 0.0771 (6) & 0.1245 (5) & \textbf{0.2847 (1)} & 0.2132 (4) & 0.2570 (2) & 0.2140 (3) & 0.0761 (6) & 0.1472 (5) & \textbf{0.3013 (1)} \tabularnewline
yeast1458v7     & \textbf{0.1433 (1)} & 0.0250 (6.0) & 0.1123 (3) & 0.1033 (4) & 0.1189 (2) & 0.0450 (5.0) & 0.0947 (2) & 0.0461 (6) &\textbf{ 0.0992 (1)} & 0.0861 (3) & 0.0793 (4) & 0.0769 (5) & 0.1045 (2) & 0.0250 (5) & \textbf{0.1193 (1)} & 0.0891 (3) & 0.0863 (4) & 0.0200 (6) \tabularnewline
abalone9-18     & \textbf{0.3203 (1)} & 0.0836 (6.0) & 0.1978 (3) & 0.1339 (5) & 0.2223 (2) & 0.1479 (4.0) & 0.2978 (3) & \textbf{0.3540 (1)} & 0.1945 (5) & 0.1307 (6) & 0.2055 (4) & 0.3460 (2) & 0.3650 (3) & \textbf{0.4101 (1)} & 0.2316 (5) & 0.1323 (6) & 0.2968 (4) & 0.3882 (2) \tabularnewline
ecoli4          & \textbf{0.8770 (1)} & 0.8571 (3.0) & 0.5377 (5) & 0.3148 (6) & 0.5533 (4) & 0.8587 (2.0) & 0.4124 (5) & \textbf{0.6760 (1)} & 0.4292 (3) & 0.3160 (6) & 0.4177 (4) & 0.6419 (2) & 0.4898 (3) & \textbf{0.6698 (1)} & 0.4739 (4) & 0.3405 (6) & 0.4362 (5) & 0.6664 (2) \tabularnewline
led02456789v1   & \textbf{0.5000 (1)} & 0.4300 (4.0) & 0.4402 (3) & 0.4072 (6) & 0.4249 (5) & 0.4467 (2.0) & \textbf{0.4065 (1)} & 0.1675 (6) & 0.2702 (5) & 0.3102 (2) & 0.2803 (3) & 0.2758 (4) & \textbf{0.4325 (1)} & 0.1286 (6) & 0.3180 (4) & 0.3141 (5) & 0.3794 (2) & 0.3397 (3) \tabularnewline
page-blocks0    & 0.7229 (3) & \textbf{0.7586 (1.0)} & 0.6823 (4) & 0.1968 (6) & 0.4094 (5) & 0.7542 (2.0) & 0.7600 (3) & 0.8123 (2) & 0.7456 (4) & 0.2099 (6) & 0.5047 (5) & \textbf{0.8248 (1) }& 0.7943 (3) & \textbf{0.8584 (1)} & 0.7534 (4) & 0.2101 (6) & 0.5066 (5) & 0.8499 (2) \tabularnewline
ecoli3          & 0.6205 (2) & 0.5905 (3.0) & 0.5540 (5) & 0.3670 (6) & 0.5748 (4) & \textbf{0.6305 (1.0)} & 0.5047 (4) & \textbf{0.5728 (1)} & 0.4843 (5) & 0.3971 (6) & 0.5471 (3) & 0.5644 (2) & 0.5464 (4) & 0.5821 (3) & 0.5441 (5) & 0.4164 (6) & 0.5914 (2) & \textbf{0.6206 (1)} \tabularnewline
yeast3          & 0.7140 (3) & 0.7225 (2.0) & 0.6569 (4) & 0.3550 (6) & 0.6568 (5) & \textbf{0.7378 (1.0)} & 0.6148 (5) & 0.6872 (2) & 0.6608 (3) & 0.4316 (6) & 0.6257 (4) & \textbf{0.7277 (1)} & 0.6855 (5) & 0.7107 (3) & 0.7175 (2) & 0.4518 (6) & 0.6897 (4) & \textbf{0.7673 (1)} \tabularnewline
new-thyroid1    & \textbf{0.8712 (1)} & 0.8147 (5.0) & 0.8635 (3) & 0.5276 (6) & 0.8268 (4) & 0.8672 (2.0) & 0.8669 (2) & 0.8228 (4) & \textbf{0.8692 (1)} & 0.6110 (6) & 0.8448 (3) & 0.8226 (5) & 0.8571 (3) & 0.8511 (4) & \textbf{0.8922 (1)} & 0.6222 (6) & 0.8608 (2) & 0.8340 (5) \tabularnewline
new-thyroid2    & 0.7783 (5) & 0.7934 (4.0) & 0.8041 (2) & 0.5129 (6) & 0.7953 (3) & \textbf{0.8154 (1.0)} & 0.8346 (2) & \textbf{0.8669 (1)} & 0.7964 (4) & 0.6337 (6) & 0.7924 (5) & 0.8325 (3) & 0.8651 (4) & \textbf{0.9003 (1)} & 0.8795 (3) & 0.6328 (6) & 0.7877 (5) & 0.8931 (2) \tabularnewline
vehicle3        & 0.5162 (4) & 0.4233 (6.0) & 0.5309 (3) & \textbf{0.5576 (1)} & 0.5099 (5) & 0.5455 (2.0) & 0.6088 (2) & 0.5411 (6) & 0.5668 (3) & \textbf{0.6097 (1)} & 0.5499 (5) & 0.5653 (4) & \textbf{0.6303 (1)} & 0.4735 (6) & 0.5870 (5) & 0.6302 (2) & 0.5890 (4) & 0.6249 (3) \tabularnewline
vehicle1        & \textbf{0.5680 (1)} & 0.4669 (6.0) & 0.5483 (5) & 0.5632 (2) & 0.5588 (3) & 0.5582 (4.0) & \textbf{0.5990 (1)} & 0.5031 (6) & 0.5469 (4) & 0.5834 (3) & 0.5205 (5) & 0.5953 (2) & \textbf{0.6161 (1)} & 0.4964 (6) & 0.6014 (4) & 0.6151 (2) & 0.5838 (5) & 0.6083 (3) \tabularnewline
vehicle2        & 0.7883 (2) & \textbf{0.8132 (1.0)} & 0.7390 (5) & 0.6918 (6) & 0.7738 (4) & 0.7852 (3.0) & \textbf{0.9095 (1)} & 0.9020 (2) & 0.8567 (5) & 0.7732 (6) & 0.8700 (4) & 0.8994 (3) & 0.9217 (2) & \textbf{0.9261 (1)} & 0.9125 (4) & 0.7849 (6) & 0.8861 (5) & 0.9142 (3) \tabularnewline
glass0          & \textbf{0.7113 (1)} & 0.6806 (4.0) & 0.6920 (3) & 0.6527 (6) & 0.6549 (5) & 0.7071 (2.0) & 0.7282 (2) & \textbf{0.7732 (1)} & 0.7087 (4) & 0.6519 (6) & 0.6533 (5) & 0.7202 (3) & 0.7331 (3) & 0.7682 (2) & \textbf{0.7776 (1)} & 0.6477 (6) & 0.6928 (5) & 0.7302 (4) \tabularnewline
pima            & \textbf{0.6527 (1) }& 0.5541 (6.0) & 0.6318 (4) & 0.6508 (2) & 0.6284 (5) & 0.6505 (3.0) & 0.4567 (2) & 0.3497 (6) & 0.3978 (4) & \textbf{0.4764 (1)} & 0.3869 (5) & 0.4476 (3) & 0.4675 (2) & 0.2823 (6) & 0.4309 (4) & \textbf{0.4735 (1)} & 0.4006 (5) & 0.4646 (3) \tabularnewline
glass1          & 0.7112 (5) & 0.7208 (3.0) & 0.7143 (4) & 0.7039 (6) & \textbf{0.7489 (1)} & 0.7298 (2.0) & \textbf{0.6650 (1)} & 0.5956 (5) & 0.6308 (3) & 0.5683 (6) & 0.6251 (4) & 0.6320 (2) & \textbf{0.6676 (1)} & 0.6617 (2) & 0.6560 (5) & 0.5856 (6) & 0.6562 (4) & 0.6579 (3) \tabularnewline
wdbc            & 0.8816 (4) & 0.8875 (3.0) & \textbf{0.8927 (1)} & 0.8775 (5) & 0.8901 (2) & 0.8756 (6.0) & \textbf{0.9118 (1)} & 0.9081 (2) & 0.8952 (4) & 0.8660 (6) & 0.8939 (5) & 0.9035 (3) & 0.9248 (4) & \textbf{0.9369 (1)} & 0.9302 (2) & 0.8898 (6) & 0.9209 (5) & 0.9260 (3) \tabularnewline
spam            & \textbf{0.7497 (1)} & 0.7391 (6.0) & 0.7406 (5) & 0.7471 (2) & 0.7436 (3) & 0.7430 (4.0) & \textbf{0.8842 (1)} & 0.8799 (2) & 0.8681 (4) & 0.8333 (6) & 0.8714 (3) & 0.8600 (5) & \textbf{0.9229 (1)} & 0.9118 (4) & 0.9194 (2) & 0.8692 (6) & 0.9158 (3) & 0.8963 (5) \tabularnewline
\hline
Avg. rank                & 2.05       & 4.17         & 3.71       & 4.76       & 3.48       & 2.83         & 2.33       & 2.95       & 3.76       & 5.00       & 4.19       & 2.76       & 2.67       & 2.95       & 3.29       & 5.14       & 4.05       & 2.90       \tabularnewline
\hline 
\end{tabular}



==> RWMaU_ICONIP2021 Paper/tables/pvals_wlt_table_aucbag_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021
\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
  RWMaU &     & 12/9/0 & 12/9/0 & 19/2/0 & 14/7/0 & 16/5/0 \\ 
  original & 0.2187 &     & 8/13/0 & 17/4/0 & 12/9/0 & 9/12/0 \\ 
  RUS & 0.6160 & 0.4608 &     & 15/6/0 & 16/5/0 & 13/8/0 \\ 
  IHT & 0.0003 *** & 0.0250 ** & 0.0015 *** &     & 4/17/0 & 5/16/0 \\ 
  CC & 0.0930 * & 0.5894 & 0.2082 & 0.0930 * &     & 9/12/0 \\ 
  NCR & 0.2003 & 0.8690 & 0.3937 & 0.0308 ** & 0.6461 &     \\ 
   \hline
\end{tabular}


==> RWMaU_ICONIP2021 Paper/tables/pvals_wlt_table_aucnor_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 20/1/0 & 17/4/0 & 19/2/0 & 18/3/0 & 21/0/0 \\ 
  original & 0.0000 *** &     & 6/15/0 & 12/9/0 & 6/15/0 & 7/14/0 \\ 
  RUS & 0.0089 *** & 0.0481 ** &     & 16/5/0 & 11/10/0 & 13/8/0 \\ 
  IHT & 0.0000 *** & 0.7051 & 0.0206 ** &     & 5/16/0 & 6/15/0 \\ 
  CC & 0.0064 *** & 0.0645 * & 0.8690 & 0.0284 ** &     & 13/8/0 \\ 
  NCR & 0.0002 *** & 0.3409 & 0.3223 & 0.1992 & 0.3617 &     \\ 
   \hline
\end{tabular}



==> RWMaU_ICONIP2021 Paper/tables/pvals_wlt_table_aucnor_knn.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 16/5/0 & 18/3/0 & 18/3/0 & 17/4/0 & 17/4/0 \\ 
  original & 0.0113 ** &     & 11/10/0 & 14/7/0 & 12/9/0 & 7/14/0 \\ 
  RUS & 0.0054 *** & 0.7900 &     & 14/7/0 & 7/14/0 & 11/10/0 \\ 
  IHT & 0.0000 *** & 0.1776 & 0.2917 &     & 5/16/0 & 7/14/0 \\ 
  CC & 0.0247 ** & 0.7594 & 0.6009 & 0.0952 * &     & 11/10/0 \\ 
  NCR & 0.0188 ** & 0.8261 & 0.6773 & 0.1198 & 0.8690 &     \\ 
   \hline
\end{tabular}


==> RWMaU_ICONIP2021 Paper/tables/pvals_wlt_table_f1bag_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 9/12/0 & 13/8/0 & 20/1/0 & 17/4/0 & 11/10/0 \\ 
  original & 0.6732 &     & 11/10/0 & 16/5/0 & 12/9/0 & 13/8/0 \\ 
  RUS & 0.3937 & 0.6454 &     & 18/3/0 & 15/6/0 & 6/15/0 \\ 
  IHT & 0.0003 *** & 0.0008 *** & 0.0049 *** &     & 4/17/0 & 5/16/0 \\ 
  CC & 0.0494 ** & 0.1198 & 0.2917 & 0.1198 &     & 5/16/0 \\ 
  NCR & 0.7051 & 0.9343 & 0.6213 & 0.0008 *** & 0.1152 &     \\ 
   \hline
\end{tabular}


==> RWMaU_ICONIP2021 Paper/tables/pvals_wlt_table_f1nor_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 12/9/0 & 15/6/0 & 19/2/0 & 17/4/0 & 14/7/0 \\ 
  original & 0.3409 &     & 14/7/0 & 16/5/0 & 14/7/0 & 11/10/0 \\ 
  RUS & 0.0395 ** & 0.2313 &     & 16/5/0 & 14/7/0 & 4/17/0 \\ 
  IHT & 0.0001 *** & 0.0019 *** & 0.0673 * &     & 5/16/0 & 4/17/0 \\ 
  CC & 0.0049 *** & 0.0673 * & 0.5066 & 0.2313 &     & 4/17/0 \\ 
  NCR & 0.5066 & 0.7415 & 0.1349 & 0.0008 *** & 0.0395 ** &     \\ 
   \hline
\end{tabular}


==> RWMaU_ICONIP2021 Paper/tables/pvals_wlt_table_f1nor_knn.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & proposed & original & RUS & IHT & CC & NCR \\ 
  \hline
proposed &     & 14/7/0 & 17/4/0 & 20/1/0 & 18/3/0 & 14/7/0 \\ 
  original & 0.0018 *** &     & 7/14/0 & 13/8/0 & 8/13/0 & 3/17/1 \\ 
  RUS & 0.0145 ** & 0.4558 &     & 16/5/0 & 9/12/0 & 5/16/0 \\ 
  IHT & 0.0000 *** & 0.3402 & 0.1265 &     & 4/17/0 & 8/13/0 \\ 
  CC & 0.0395 ** & 0.3019 & 0.6801 & 0.0548 * &     & 8/13/0 \\ 
  NCR & 0.2487 & 0.0515 * & 0.2026 & 0.0042 *** & 0.3200 &     \\ 
   \hline
\end{tabular}


==> tables/ds_description_transpose.tex <==
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrr}
  \hline
 & new-thyroid1 & pima & yeast4 & glass1 & vehicle3 & glass0 & ecoli3 & ecoli4 & vehicle1 & wdbc & new-thyroid2 & yeast1458v7 & yeast5 & yeast3 & vehicle2 & abalone9-18 & led02456789v1 & page-blocks0 & spam & yeast1289v7 & wine-red-4 \\ 
  \hline
n & 215.00 & 768.00 & 1484.00 & 214.00 & 846.00 & 214.00 & 336.00 & 336.00 & 846.00 & 569.00 & 215.00 & 693.00 & 1484.00 & 1484.00 & 846.00 & 731.00 & 443.00 & 5472.00 & 4597.00 & 947.00 & 1599.00 \\ 
  d & 5.00 & 8.00 & 8.00 & 9.00 & 18.00 & 9.00 & 7.00 & 7.00 & 18.00 & 30.00 & 5.00 & 8.00 & 8.00 & 8.00 & 18.00 & 8.00 & 7.00 & 10.00 & 57.00 & 8.00 & 11.00 \\ 
  imb.ratio & 5.14 & 1.87 & 28.10 & 1.82 & 2.99 & 2.06 & 8.60 & 15.80 & 2.90 & 1.68 & 5.14 & 22.10 & 32.73 & 8.10 & 2.88 & 16.40 & 10.97 & 8.79 & 1.54 & 30.57 & 29.17 \\ 
   \hline
\end{tabular}


==> tables/pvals_wlt_table_aucbag_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021
\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
  RWMaU &     & 12/9/0 & 12/9/0 & 19/2/0 & 14/7/0 & 16/5/0 \\ 
  original & 0.2187 &     & 8/13/0 & 17/4/0 & 12/9/0 & 9/12/0 \\ 
  RUS & 0.6160 & 0.4608 &     & 15/6/0 & 16/5/0 & 13/8/0 \\ 
  IHT & 0.0003 *** & 0.0250 ** & 0.0015 *** &     & 4/17/0 & 5/16/0 \\ 
  CC & 0.0930 * & 0.5894 & 0.2082 & 0.0930 * &     & 9/12/0 \\ 
  NCR & 0.2003 & 0.8690 & 0.3937 & 0.0308 ** & 0.6461 &     \\ 
   \hline
\end{tabular}


==> tables/pvals_wlt_table_aucnor_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 20/1/0 & 17/4/0 & 19/2/0 & 18/3/0 & 21/0/0 \\ 
  original & 0.0000 *** &     & 6/15/0 & 12/9/0 & 6/15/0 & 7/14/0 \\ 
  RUS & 0.0089 *** & 0.0481 ** &     & 16/5/0 & 11/10/0 & 13/8/0 \\ 
  IHT & 0.0000 *** & 0.7051 & 0.0206 ** &     & 5/16/0 & 6/15/0 \\ 
  CC & 0.0064 *** & 0.0645 * & 0.8690 & 0.0284 ** &     & 13/8/0 \\ 
  NCR & 0.0002 *** & 0.3409 & 0.3223 & 0.1992 & 0.3617 &     \\ 
   \hline
\end{tabular}



==> tables/pvals_wlt_table_aucnor_knn.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 16/5/0 & 18/3/0 & 18/3/0 & 17/4/0 & 17/4/0 \\ 
  original & 0.0113 ** &     & 11/10/0 & 14/7/0 & 12/9/0 & 7/14/0 \\ 
  RUS & 0.0054 *** & 0.7900 &     & 14/7/0 & 7/14/0 & 11/10/0 \\ 
  IHT & 0.0000 *** & 0.1776 & 0.2917 &     & 5/16/0 & 7/14/0 \\ 
  CC & 0.0247 ** & 0.7594 & 0.6009 & 0.0952 * &     & 11/10/0 \\ 
  NCR & 0.0188 ** & 0.8261 & 0.6773 & 0.1198 & 0.8690 &     \\ 
   \hline
\end{tabular}


==> tables/pvals_wlt_table_f1bag_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 9/12/0 & 13/8/0 & 20/1/0 & 17/4/0 & 11/10/0 \\ 
  original & 0.6732 &     & 11/10/0 & 16/5/0 & 12/9/0 & 13/8/0 \\ 
  RUS & 0.3937 & 0.6454 &     & 18/3/0 & 15/6/0 & 6/15/0 \\ 
  IHT & 0.0003 *** & 0.0008 *** & 0.0049 *** &     & 4/17/0 & 5/16/0 \\ 
  CC & 0.0494 ** & 0.1198 & 0.2917 & 0.1198 &     & 5/16/0 \\ 
  NCR & 0.7051 & 0.9343 & 0.6213 & 0.0008 *** & 0.1152 &     \\ 
   \hline
\end{tabular}


==> tables/pvals_wlt_table_f1nor_c45.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & RWMaU & original & RUS & IHT & CC & NCR \\ 
  \hline
RWMaU &     & 12/9/0 & 15/6/0 & 19/2/0 & 17/4/0 & 14/7/0 \\ 
  original & 0.3409 &     & 14/7/0 & 16/5/0 & 14/7/0 & 11/10/0 \\ 
  RUS & 0.0395 ** & 0.2313 &     & 16/5/0 & 14/7/0 & 4/17/0 \\ 
  IHT & 0.0001 *** & 0.0019 *** & 0.0673 * &     & 5/16/0 & 4/17/0 \\ 
  CC & 0.0049 *** & 0.0673 * & 0.5066 & 0.2313 &     & 4/17/0 \\ 
  NCR & 0.5066 & 0.7415 & 0.1349 & 0.0008 *** & 0.0395 ** &     \\ 
   \hline
\end{tabular}


==> tables/pvals_wlt_table_f1nor_knn.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Sun Jun 20 22:20:37 2021

\begin{tabular}{lllllll}
  \hline
 & proposed & original & RUS & IHT & CC & NCR \\ 
  \hline
proposed &     & 14/7/0 & 17/4/0 & 20/1/0 & 18/3/0 & 14/7/0 \\ 
  original & 0.0018 *** &     & 7/14/0 & 13/8/0 & 8/13/0 & 3/17/1 \\ 
  RUS & 0.0145 ** & 0.4558 &     & 16/5/0 & 9/12/0 & 5/16/0 \\ 
  IHT & 0.0000 *** & 0.3402 & 0.1265 &     & 4/17/0 & 8/13/0 \\ 
  CC & 0.0395 ** & 0.3019 & 0.6801 & 0.0548 * &     & 8/13/0 \\ 
  NCR & 0.2487 & 0.0515 * & 0.2026 & 0.0042 *** & 0.3200 &     \\ 
   \hline
\end{tabular}

